Caching at the Edge: Outage Probability

Caching at the edge of wireless networks is a keytechnology to reduce traffic in the backhaul link. However, aconcentrated amount of requests during peak-periods may causethe outage of the system, meaning that the network is not ableto serve the whole set of demands. The outage probability is afundamental metric to take into account during the networkdesign. In this paper, we derive the analytical expression ofthe outage probability as a function of the total amount ofusers requests, library size, requests distribution, cache size andcapacity constraints on the backhaul resources. In particular, wefocus on a scenario where end-users have no direct connectionto the master node which holds the complete library of contentthat can be requested. A general formulation of the outage isderived and studied for two relevant caching schemes, i.e. therandom caching scheme and the most popular caching schemes.The exact closed form expressions presented in this paper provideuseful insights on how requests, memory and resources can bebalanced when the parameters of a cache-enabled network haveto designed

==> 0_Aux/notation.tex <==
\newcommand{\source}{\mathcal{S}}
\newcommand{\library}{\mathcal{F}}
\newcommand{\nfiles}{N}


\newcommand{\relayset}{\mathcal{H}}
\newcommand{\relay}{h}
\newcommand{\nusers}{d}
\newcommand{\nactive}{u_d}
\newcommand{\cachesize}{M}

\newcommand{\capacity}{C}
\newcommand{\probrelay}[1]{\gamma_{#1}}

\newcommand{\Pout}{\ensuremath{\mathsf{P_{out}}}}
\newcommand{\Ps}{\ensuremath{\mathsf{P_{succ}}}}
\newcommand{\Pnot}{\ensuremath{\mathsf{P_{nc}}}}



\newcommand{\Pp}{\mathsf{P}}
\newcommand{\Pc}{\mathsf{P_c}}
\newcommand{\Pm}{\mathsf{P_M}}
\newcommand{\Pk}{p_{\Kreq}}
\newcommand{\Plam}{\mathsf{P_{\Lambda}}}
\newcommand{\Zdiff}{\ensuremath{\mathsf{Z}}}
\newcommand{\zd}{\mathsf{z}}

\newcommand{\Kreq}{\ensuremath{\mathsf{K}}}
\newcommand{\kr}{\mathsf{k}}




\newcommand{\Pu}{\mathsf{P_U}}
\newcommand{\J}{\mathsf{J}}

\newcommand{\Psuc}{\mathsf{P_{B|J}}}
\newcommand{\Pcache}{\mathsf{P_{J}}}
\newcommand{\libraryf}[1]{\mathsf{f}_{#1}}



\newcommand{\area}[1]{a_{#1}}





\newcommand{\estef}{\textcolor{black}}
\newcommand{\change}{\textcolor{orange}}


==> 0_Aux/packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{amsmath,amsthm,graphicx,cite}
\usepackage{epsfig,amsfonts}
\usepackage{graphicx,cite,amssymb,amsmath}
\usepackage{color}
%\usepackage{caption}
\usepackage{enumitem}
\usepackage{dblfloatfix}
\usepackage[nolist]{acronym}
\usepackage{psfrag}
% \usepackage{perso}
%\usepackage{blindtext}
\usepackage[keeplastbox]{flushend}
%\usepackage[paperheight=9.7cm,paperwidth=10.1cm,margin=0.10cm,heightrounded]{geometry}
%\usepackage{relsize}
\usepackage{mathtools}
\mathtoolsset{showonlyrefs}
%\usepackage{flushend}
\usepackage{placeins}

%\ifCLASSOPTIONcompsoc
%\usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%\usepackage[caption=false,font=footnotesize]{subfig}
%\fi
%
%\usepackage[font=small,labelfont=bf]{caption}

 % \linespread{1.12}


==> 0_Aux/title.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
\title{     Caching  at the Edge: Outage Probability}

\author{
   \IEEEauthorblockN{Estefan\'ia Recayte, Andrea Munari\\
    \IEEEauthorblockA{\IEEEauthorrefmark{1}Institute of Communications and Navigation of DLR (German Aerospace Center),
 \\Wessling, Germany. Email:  \{estefania.recayte, andrea.munari\}@dlr.de}\\
 }
}
\maketitle


%\maketitle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%
%\tableofcontents

%\thispagestyle{empty}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
% \thispagestyle{empty} \pagestyle{empty}


\begin{abstract}
Caching at the edge of wireless networks is a key technology to reduce traffic in the backhaul link. However, a concentrated amount of requests during peak-periods may cause the outage of the system, meaning that the network is not able to serve the whole set of demands.  The outage probability is a fundamental metric to take into account during the network design. In this paper,  we derive  the analytical expression of the outage probability as a function of the total amount of users requests, {library size}, requests distribution, cache size and capacity constraints on the backhaul resources. In particular, we focus on a scenario where end-users have no direct connection to the master node which holds the complete library of content that can be requested. A  general formulation of the outage is derived and   studied for two relevant caching schemes, i.e. the random caching scheme and the most popular caching schemes. The exact closed form expressions presented in this paper provide useful insights on how requests, memory and resources can be balanced when the parameters of a cache-enabled network have to   designed.
\end{abstract}

\vspace{1cm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{keywords}
%\end{keywords}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

